CLIPGraphs: Multimodal Graph Networks to Infer Object-Room Affinities

This paper introduces a novel method for determining the best room to place an object in, for embodied scene rearrangement. While state-of-the-art approaches rely on large language models (LLMs) or reinforcement learned (RL) policies for this task, our approach, CLIPGraphs, efficiently combines commonsense domain knowledge, data-driven methods, and recent advances in multimodal learning. Specifically, it (a)encodes a knowledge graph of prior human preferences about the room location of different objects in home environments, (b) incorporates vision-language features to support multimodal queries based on images or text, and (c) uses a graph network to learn object-room affinities based on embeddings of the prior knowledge and the vision-language features. We demonstrate that our approach provides better estimates of the most appropriate location of objects from a benchmark set of object categories in comparison with state-of-the-art baselines

==> sections/ablations.tex <==
\section{Appendix}\label{section:ablations}

\textbf{[Thoughts]} We also plan to discuss a bit about the High-Level category mAP of various baselines. So from \ref{table:final-comparison}, we get 3 plots of High Level mAP's. Before showing that we also plan to tell them what are the various high level categories\cite{Kant2022HousekeepTV} 
We then show the confusion matrix of the best GCN + CLIP finetuned model

\subsection{Loss Function}
\subsubsection{Structure}

The spine of our training lies in the efficacy of our loss function. There have been various experiments with what works well for Representation Learning [cite some papers]. However with the recent success of CLIP-Field's Formulation of Contrastive Loss \cite{CLIP-Fields} we choose this as the skeleton for our loss function ablations. Here for each batch they take 1 anchor, 1 positive node wrt to that anchor, and $k$ negative nodes wrt to that anchor. We run ablations on $batch\ size$ as well as $k$ and tune the $temp$ hyperparameter on the validation set. 

\subsubsection{Sampling}
The benefits of $k$ negatives over the traditional triplet loss\cite{Schultz2003LearningAD} are intuitive as well as have been sufficiently well proven in the literature. [cite plz]. Thus we directly begin with our ablation results. For our sampling and batch size ablations, we keep the $temp$ as 0.01. Once we got the best batch size and sampling parameters, we tuned our $temp$ hyperparameter to maximize mAP over the validation set. We get it as $0.01$ 

\textcolor{red}{add the plots for Vit vs RN50 vs COnvNext for batch size , k, sampling technique, temp =0.01}
\subsubsection{Comments}

\begin{itemize}
    \item batch size, circumventing the  room bias 
\end{itemize}



\subsection{Loss Function Ablations}
\begin{itemize}
    \item  L2 : single +ve \& k negative
    \item   k negatives , batch size, edge weight vs no edge weight, norm edge weight vs unnorm edge weight, usage of edge weights
\end{itemize}
\subsection{Hyperparameter Tuning Plots}

\begin{figure}[tb]
    \centering
        \includegraphics[width=0.5\textwidth]{sections/figures/loss_curve.png}
    \caption[Loss Curve]{Convergence of the Loss Curve}
    \label{fig:loss}
\end{figure}

\begin{table}[h]
\centering
\begin{tabular}{lll}
\hline
\# & \textbf{Hyperparameter} & \textbf{Value} \\
\hline
1 & Node Feature Size & 1024(ViT) / 512 (Others) \\
2 & Output Node Embedding & 128 \\
3 & GCN Layers &  \\
4 & Learning Rate &  \\
5 & Learning Rate Schedule & \\
6 & Temperature & \\
7 & Batch Size [Loss] &  \\
8 & Negatives Per Batch &  \\
9 & Sampling Method &  \\
\hline
\end{tabular}
\caption{Hyperparameter choices for fine-tuning CLIP Visual Encoder Features on our GCN}
\label{table:hyp}
\end{table}

We tried initializing the room node features as 1-hot features, random and corresponding to the CLIP Language Encoders but everytime our training converged to the same point and gave us the same Test mAP. Thus we can safely conclude that the room node features don't affect the performance

% \subsection{Discussions on Housekeep Dataset}\label{section:ablations-discuss-HK}
% \begin{itemize}
%     % \item Its misbalanced nature and the missing step of room ranking from their data collection pipeline. This was because they were more focused on getting ORR ranks. For example, their ground truth data said the correct room for 'banana' is a 'garage'.

%     % \item We need some good ways to explain RRC Commonsense Object Room Mappings; either we say that we used ChatGPT to give us ground truth mappings and we use the housekeep ranks to assign the soft scores [edge weights in our graph]. But we lose a baseline comparison if we say this\\
%     % We discuss how we overcame the bias of the dataset and got new annotators who focussed on giving us their preference for Object-Room mappings. We show the results of our survey and then proceed to bash Housekeep GT

    
% \end{itemize}

\subsection{More About Graph Creation}

\begin{itemize}
    \item Getting Object-Room GT Relationships on the basis of human annotations. A journey from human ranks to soft score. And further till OR Ground truths.
\end{itemize}

\subsection{Are these figures needed?}
Figures \ref{fig:ablation} and \ref{fig:loss}
, figure comparing training and validation mAPs?

%------------------------------------------------------------
\begin{figure}[tb]
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{sections/figures/batch.png}
        \caption{Ablation on batch-sizes with test mAP.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{sections/figures/neg_samples.png}
        \caption{Ablation on the number of negative samples in the contrastive loss.}
    \end{subfigure}
    \caption[Ablations]{Ablations. Needed? Change the scale of x-axis to linear?}
    \label{fig:ablation}
\end{figure}
%---------------------------------------------------------

%------------------------------------------------------------

%---------------------------------------------------------

\begin{figure*}[tb]
    \centering
        \includegraphics[width=0.7\textwidth]{sections/figures/gandr-collage.jpg}
    \caption{Representative Image Of Our Web Scraped Dataset ; 1 image per object category}
    \label{fig:dataset-collage}
\end{figure*}

\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
\textbf{Statistics About our Knowledge Graph } & \textbf{Value} \\
\hline
\#Nodes & {4020 Object Images Nodes \& 17 Room Nodes}\\
\#Edges &  7,66,649\\
Self Loops & Yes \\
Train Images & 268*15 Images \\
Test Images & 268*10 Images\\
Val Images & 268*5 Images\\
Types of edges & weighted undirected \\
\hline
\end{tabular}
\caption{Statistics for the Knowledge Graph created using the web scraped dataset}
\label{table:graph-stats}
\end{table}

\begin{figure*}[htbp]
  \centering
  \begin{minipage}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{sections/figures/tsne-1.png}
    \caption{Untrained TSNE}
    \label{fig:untrained-tsne}
  \end{minipage}\\
  \hspace{0.5cm}
  \begin{minipage}[b]{\linewidth}
    \includegraphics[width=\linewidth]{sections/figures/tsne-f.png}
    \caption{t-SNE visualization of our embeddings on the test split of the Web Scraped Dataset\ref{section:datasets-web}. The boxes are representative of the type of images getting clustered.}
    \label{fig:clustered-tsne}
  \end{minipage}
\end{figure*}

==> sections/datasets.tex <==
\section{Datasets}
\subsection{Datasets}
\subsubsection{Housekeep Human Annotations}\label{HGT}
Housekeep\cite{Kant2022HousekeepTV} generated a human preference dataset using Amazon MTurk \cite{crowston2012amazon} with 372 human annotators. The annotators ranked each receptacle under the `correct', `misplaced', and `implausible' categories. We convert these ranks into soft scores for each object-room-receptacle pair using mean reciprocal rank for correct and misplaced categories. [see \ref{section:ablations}] These scores are used to assign edge weights to the graph. 

\subsubsection{IRONA(Image Recognition Object Names and Annotations) Web-Scraped Dataset}\label{section:datasets-web}
To create a visual dataset that corresponds to the Housekeep\cite{Kant2022HousekeepTV} Object Names, we followed the same object categories as the original paper. For each of the 268 object categories, we scraped the web for 30 images that represent the objects in different settings and perspectives. This resulted in a dataset of 8040 images that can be used to train and test our models on visual commonsense reasoning in the home.

% \subsubsection{Visual Housekeep Dataset}\label{section:datasets-visualhk}
% We also evaluate our models on another visual dataset that we create by taking 2-D snapshots of the 3-D models of the objects used by Housekeep \cite{Kant2022HousekeepTV} rearrangement simulation episodes. 

% \subsubsection{RRC Real-Objects Dataset}
% To compare our model on real-world noisy images and in presence of background objects we create a new dataset where we click photos from a mobile phone [Specifications to be added]. We recreate some common shortcomings in Real World Transfer of Vision-Guided Embodied AI agents. These included Flash photograp[hy in a dark room, overexposure, graining in the image, black/white ]

\subsection{Graph Creation}
\input{sections/graph_creation}

==> sections/graph_creation.tex <==
% \section{Making Sense of Data: Graph Creation}
For our experiments, we utilized the IRONA web-scraped dataset which consists of web-scraped images for 268 object categories. The dataset was partitioned into training, validation and testing sets in a ratio of 15:5:10 images per object category. To maintain uniformity we've maintained the same High-Level Classification of objects into categories like apparel, packaged food, etc.  We use the human annotation ranks by Housekeep \cite{Kant2022HousekeepTV} where for every object-room pair, 10 human annotators have ranked the receptacles present in that room on the basis of the likelihood of each object to be placed in a correct and misplaced sense. Thus, for each Object-Room-Receptacle tuple, there would be 10 opinions which could be either +ve/-ve or zero. We obtain the filtered data where only 8/10 such opinions are registered so that there is a good agreement amongst the annotators. We then calculate both positive soft scores and negative soft scores by calculating a mean of the positive reciprocal ranks and negative reciprocal ranks respectively over all the receptacles for a given object-room pair. We guide the interested readers to \ref{section:ablations} For a given object; to create a Ground Truth mapping for top-k correct Object-Room mappings; We use the object-room-receptacle scores by selecting the room containing the highest positive-scored receptacle. Every other room is mapped to this object using the mean negative soft score of each receptacle belonging to the room.

Once we get the mapping weight of each Object-Room connection; we use this to populate a knowledge graph. We instantiate the training graph with each image of the training split as a node. We also add nodes corresponding to Room Names. So we have 268*15 + 17 = 4037 nodes. \\
To add edges to connect these nodes we use $5$ type of edges (as shown in figure \ref{figure:edges}):
\begin{enumerate} 
    \item Image Self Edge (edge weight=1)
    \item Edge between same object's 2 images (edge weight= rand(0.5-0.7))
    \item Edge between 2 objects that belong to same GT Room 
    \item Edge between image and that object's correct GT Room Node
    \item Edge between image and that object's incorrect GT Room Nodes
\end{enumerate}

\begin{figure}[tb] 
        \centering     
        \includegraphics[width=0.45\textwidth]{sections/figures/edge-2.png}
        \caption{An illustration to show 5 types of edges. The colored edges denote positive edge weights whereas black ones denote negative. The number on the edges denote the type of edge to which they belong}
        \label{figure:edges}
\end{figure}

Corresponding to these 5 types of edges, we assign each of them some edge weights. Edge weights for Type 4,5 are obtained from the Object Room Soft Scores. Type 3 is being given an edge weight of a fraction randomly chosen between 0.5 to 0.7, while for Type1,2 we assign them edge weights of 1. \newline
% \href{https://drive.google.com/file/d/1cuxPt4U7uU14QN15CTMe6Ex7pk4OuAT5/view?usp=sharing}{link}
Our graph contains CLIP Image Encoder Features as node features for images of 268 objects, and CLIP Language Encoder Features for 17 rooms. \newline 




